Online Myopic Network Covering

Efficient marketing or awareness-raising campaigns seek to recruit $n$ influential individuals -- where $n$ is the campaign budget -- that are able to cover a large target audience through their social connections. So far most of the related literature on maximizing this network cover assumes that the social network topology is known. Even in such a case the optimal solution is NP-hard. In practice, however, the network topology is generally unknown and needs to be discovered on-the-fly. In this work we consider an unknown topology where recruited individuals disclose their social connections (a feature known as {\em one-hop lookahead}). The goal of this work is to provide an efficient greedy online algorithm that recruits individuals as to maximize the size of target audience covered by the campaign. We propose a new greedy online algorithm, Maximum Expected $d$-Excess Degree (MEED), and provide, to the best of our knowledge, the first detailed theoretical analysis of the cover size of a variety of well known network sampling algorithms on finite networks. Our proposed algorithm greedily maximizes the expected size of the cover. For a class of random power law networks we show that MEED simplifies into a straightforward procedure, which we denote MOD (Maximum Observed Degree). We substantiate our analytical results with extensive simulations and show that MOD significantly outperforms all analyzed myopic algorithms. We note that performance may be further improved if the node degree distribution is known or can be estimated online during the campaign.

==> RS.tex <==
%!TEX root = wwwpaper2.tex

\section{Uniform Node Sampling}
In what follows we start by violating one of our assumptions, just to show that random sampling performs poorly even under favorable conditions.
The violation is assuming that list of nodes in the target subpopulation is available.
For example this is the case of the social network VK\cite{vk}---popular among Russian speaking populations---that provides a list of all its users 
and pointers to their walls. In this case a simple network covering approach is random node uniform sampling.
Namely, we assume that each node is sampled uniformly at random and once a node is sampled we
immediately know all its neighbors. We consider both sampling with replacement and
without replacement.

We forewarn that using uniform sampling to cover a small subpopulation could be very
problematic as we shall waste a lot of samples trying to hit infrequently subpopulation
members.  

%
\subsection{With Replacement}
It is easier to analyze the sampling with replacement as it
can be described with the help of the binomial distribution.  
At each slot an uncovered node $v$ can be covered if it is sampled or if one of its 
$k_v$ neighbors is selected. This  occurs  with probability $(k_v+1)/N$.
We can then derive an analytic expression for the expected number of uncovered
nodes at time step $t$.
\begin{equation}
\label{eq:EWkReplace}
\begin{aligned}
\av{W(t)}  %& =  \sum_{v \in V} E[\bone \{\mbox{node $v$ is uncovered}\}] \\
&=\sum_{v \in V} P[\mbox{node $v$ is uncovered}]=\sum_{v \in V} \left(1-\frac{k_v+1}{N}\right)^t = \\
&= N \sum_{\forall k} p_k \left(1-\frac{k+1}{N}\right)^t,
\end{aligned}
\end{equation}
where $(p_k)_{k=1,\dots N}$ is the node degree distribution.
%Of course, the expected number of nodes covered so far is just given by
%$$
%\av{B(t) + G(t)}= N - \av{W(t)}.
%$$
For small values of $t (k_v+1)/N$, we can use the Taylor series expansion
$(1-p)^t \approx 1- t p$ 
%and the law of large numbers, 
to obtain
\begin{equation}
\label{eq:EWkReplaceApprox}
E[W(t)] \approx N - (\av{k}+1)t,
\end{equation}
where $\av{k}=\sum_{\forall v } k_v/N$ is the empirical node degree average.
%If we use the configuration network \cite{HofstadRG} to model the underlying network,
%we can express $E[W(t)]$ in a simple closed form expression. 
%Let $K$ be the degree of randomly sampled node. Then, we have
%\begin{equation}
%\begin{aligned}
%\label{eq:EWkReplaceConf}
%E[W(t)] & = N E\left[\left(1-\frac{K+1}{N}\right)^t\right] \\
%& = N \sum_{\forall k} p_k \left(1-\frac{k+1}{N}\right)^t,
%\end{aligned}
%\end{equation}
%where $\{p_k\}_{k=1,\dots}$ is the node degree distribution.

\subsection{Without Replacement}
Let us now consider the uniform node sampling without replacement.
When there is no replacement, the processes is more complicated but
we still can derive analytic approximations. 
The probability that a node uncovered until time $t-1$ is covered at time $t$ increases with $t$ as
the number of uncovered nodes reduces. If we approximate such probability with $(k_v+1)/\av{W(t-1)}$,
we can get the following formula:
\begin{equation}
\label{eq:EWkNoReplace}
\begin{aligned}
\av{W(t)} &\approx \sum_{v \in V}  \prod_{h=0}^{t-1} \left(1-\frac{k_v+1}{\av{W(h)}}\right)=\\
&= N \sum_{\forall k} p_k \prod_{h=0}^{t-1} \left(1-\frac{k+1}{\av{W(h)}}\right),
\end{aligned}
\end{equation}
where $\av{W(0)}=N$.

{\color{red} DISCUSSION.}

%The expected number of nodes which are uncovered at
%time step $t$ is given by
%\begin{equation}
%\begin{aligned}
%\av{W(t)} & = \sum_{v \in V} E[\bone{\{\mbox{node $v$ is uncovered}\}}] \nonumber \\
%& = \sum_{v \in V} P[\mbox{node $v$ is uncovered}] \nonumber
%\end{aligned}
%\end{equation}
%\begin{equation}
%\label{eq:EWkNoReplace}
%\approx \sum_{v \in V} \left(1-\frac{k_v+1}{N}\right)
%\left(1-\frac{k_v+1}{E[W(1)]}\right) \ldots \left(1-\frac{k_v+1}{E[W(t-1)]}\right)
%\end{equation}
%We note that~\eqref{eq:EWkReplace} is an upper bound
%for expression~\eqref{eq:EWkNoReplace}. Similarly to the case with
%replacement, we can obtain a closed form expression for the above expression
%in the configuration network model.
%\begin{equation}
%\begin{aligned}
%\label{eq:EWkReplaceConf}
%E[W(t)]  & = N E\left[ \prod_{h=0}^{t-1} \left(1-\frac{K+1}{E[W(h)]}\right)\right] \\
%& = N \sum_{\forall k} p_k \prod_{h=0}^{t-1} \left(1-\frac{k+1}{E[W(h)]}\right) .
%\end{aligned}
%\end{equation}


==> experiments.tex <==
\section{Experiments}




==> foundations.tex <==
\section{Understanding SI Algorithm Efficiency}\label{sec:SIDF}

SI (Poisson) epidemic as stochastic Dual Fitting algorithm for network exploration.

\subsection{Finite Graph Effect on Diffusions} \label{sec:finite}
In {\em pay-per-node} diffusions it is paramount to understand the effect that a finite graph has on {\em pay-per-node} diffusions (and diffusions in general).
In a finite graph the degree distribution of unpaid nodes may change as the diffusion progresses.
Even in the early stages of the diffusion, the degree distribution of unpaid nodes can be strikingly different than the degree distribution of the original graph.
This effect on the degree distribution of susceptible nodes of SIS and SIR epidemics has been captured in~\cite{Volz-FiniteSIS-08,Noel-FiniteEpidemic09}, respectively.
XXXXXXXX
We, however, are interested in the impact on the first order increase in cover set sizes $|\cI(n)|-|\cI(n-1)|$, $n\geq 0$.

In what follows we compute the cover set size of Markovian diffusions (a Markovian diffusion has the property that future states depend only on the current diffusion state).
SI, SIS, SIR, BFS, DFS, and RW are examples of Markovian diffusions.

\subsubsection{Random Diffusions}
\paragraph{SI}
The cover set size 

\paragraph{RW}
The cover set size 

Let us take the second order derivative
\[
\sum_v \frac{d}{dp_v}[(1-p_v)^k]_{kk} = \sum_v (1-p_v)^k \log^2(1-p_v) > 0
\]
Thus $\langle W_k \rangle$ should be strictly convex and $n-\langle W_k \rangle$ strictly concave.


(a) Ring is just a ring of $n$ nodes. In this case
\[
n-\langle W_k \rangle = n - n (1-3/n)^k
\]
(b) Star is just a star topology with one central node and n leave nodes. In this case
\[
n-\langle W_k \rangle = n - n (1 - (1+n)/(2n))^k
\]
In both cases the shape is as we would like to have it and the asymptotics for small k
is good.  In particular, for the star topology $n-\langle W_1 \rangle =(n+1)/2$ (in effect with probability $1/2$
we discover all nodes).  

\subsection{Node Degree Estimation} \label{sec:estimation}


Extend our Coupon collector approximation devised for random walks to the SI exploration problem

Crawler: Improving SI epidemic using Gibbs sampling (Stochastically choosing fitness function based on Expected uncovered degree)

If model has different types (think of belonging to clusters) of nodes, expected value may not be the best choice. One could think of adding the variance to the fitness function. Risk averse / risk prone crawlers.



==> introduction.tex <==
%!TEX root = paper.tex


\section{Introduction}
\begin{itemize}
\item General problem of budget allocation for the dominating set covering problem.
\begin{itemize}
\item FINITE GRAPH EFFECTS PLAY A BIG ROLE AND HAVE BEEN NEGLECTED. ADVERTISEMENT MIGHT TARGET A SPECIFIC COMMUNITY THAT CAN BE ``SMALL'' (Actually, even moderately large graphs suffer from finite effects. Other approaches consider infinite graphs).
\end{itemize}
\item Application ON VIRAL MARKETING
\item Application on network discovery
\item Present our results. E.g., selecting node with largest observed degree pays off in the beginning but it is detrimental by the end.
\end{itemize}
Diffusion processes crawl a network visiting nodes through their edges. 
There are a number of different types of network diffusions (and models). Viruses and Web crawlers are just two types of diffusions. 
The social network -- the graph of relationships and interactions within a group of individuals -- plays a fundamental role as a medium for the spread of information, ideas, and influence among its members.
A VARIETY OF WORKS HAVE LOOKED AT VIRAL MARKETING CAMPAINGS.
An important type of diffusion that we call {\em pay-per-node} diffusion has received little attention in the literature. 
To better understand this type of diffusion, consider  the following example.
Facebook marketeers rely on ``word-of-mouth'' advertisement to reach their costumers, also known as viral marketing campaigns~\cite{viral}.
For an ad to reach all friends of a given Facebook user it requires the user to just to post the ad on his or her {\em Facebook wall}.
Companies like Aveda (cosmetics) give incentives (discounts) to Facebook users to place adds on their walls.
The ads show discounts for users that join their viral marketing campaign (thus posting an add in their {\em Facebook wall}).
The campaign goal is to reach the most number of users given a fixed budget.

Another -- more mundane -- example of a {\em pay-per-node} diffusion is sampling online social networks (OSNs).
Researchers often do not have access to OSN databases but are allowed to crawl the OSN graph constrained by a maximum sampling rate per hour.
Each sampled user counts towards the sampling ``budget'', thus one must choose which should be the next sampled node carefully.
A greedy approach would choose the next node to be the node with the most number of connections to previously unknown nodes.
However, with rare exceptions (e.g., Google's PageRank-biased Web crawlers~\cite{GoogleCrawlers}) researchers ignore this crucial strategic sample selection problem, making a simple Breadth-First Search (BFS) the crawler of choice.
The excuse is that there is often no lookahead of node degrees, i.e., OSNs often do not publish the degree of nodes in advance, so there is no way to differentiate nodes in the selection process.
Yet another example are bot-nets. Bot-nets are centrally coordinated virus-infected zombie machines. Often used in Internet denial-of-service attacks, bot-nets can be though of a virus epidemic that is centrally coordinated.

In this work we take a principled look at {\em pay-per-node} diffusions on finite graphs.
First we show that finite graph effects must not be ignored, even for large graphs (e.g., Facebook).
We detail the precise impact of finite graph effects in the diffusion.
Our interest is focused on {\em flat-priced} pay-per-node diffusions, where the price of enrolling a node in the diffusion is the same for all nodes.
Clearly not all pay-per-node diffusions are flat-priced, for instance, viral marketing campaings may need to pay different prices for the participation of different nodes (some nodes may never join a given campaign for any price, e.g., environmentalists are unlikely to join a campaign that encourages the killing of dolphins). 

Surprisingly, studying the mechanics of next-node-visits of ``dumb'' naturally occurring diffusions such as Susceptible-Infected epidemic (SI) and Random Walks (RWs) we uncover efficient diffusion principles that can be applied to {\em pay-per-node} diffusions. 
These mechanisms outperform widely used man-made algorithms such as Breadth-First Search (BFS) and Depth-First Search (DFS). In fact, we show that DFS is as bad as it gets as a {\em pay-per-node} diffusion process. 
We also prove that the diffusion state provides enough information to estimate the average degree of next-to-visit nodes (we also present an estimator).
The latter means that even without  node degree ``lookaheads'' on can select node payments based on node degrees.

This paper is divided as follows. Section~\ref{sec:theo} presents the theoretic formulation of our problem and a couple of simple examples to illustrate some of the key points. Section~\ref{sec:}


\section{Problem Formulation}\label{sec:theo}
pay-per-node diffusions are stochastic processes that output three sequences: (1) a sequence of paid (visited) nodes $\chi(n) = \{X_i\}_{i =1}^n$, where $n$ is the $n$-th payment (node visit), and (2) a set of covered nodes $\cI(n)$ (nodes that are either paid or neighbor of a paid node). 
The cover set $\cI(n)$ is also known as the  {\em influence set} in the viral marketing campaign literature~\cite{viral}.
The algorithm that describes the selection of $X_i$ at time step $i$ is denoted {\em diffusion algorithm}. 
As algorithms, RWs and SI are highly randomized and distributed while BFS and DFS are highly centralized and deterministic.
A {\em pay-per-node} diffusion algorithm has three components:
\begin{itemize}
\item next-payment queue, where the nodes that be offered payment are stored;
\item payment scheduler selects the next node to be paid from the next-payment queue; and
\item state memory, in which the set of visited nodes already paid.
\end{itemize}

To illustrate these different components, we focus on the SI diffusion algorithm to better understand the framework. We start describing SI as a decentralized algorithm to then describe a stochastic equivalent centralized algorithm. We start with a given set of paid (infected) nodes $I$. The probability that a paid (infected) node ``infects'' an unpaid (susceptible) node during a small time interval $\Delta t > 0$ is $\beta \Delta t$, where $\beta >0$ is the infection rate. In more accurate terms, $\beta$ is a localized infection capacity parameter. The SI diffusion progresses until all nodes are infected. The above distributed version of the SI diffusion forms a Markov chain. Looking at the embedded points of the Markov chain we derive its centralized discrete-time counterpart: 
\begin{enumerate}
\item {\em State Memory:} The state memory, $\cM$, is initialized $\cM \leftarrow I$.
\item {\em Next-payment Queue:} The next-payment queue, $\cQ$, has $k_v \geq 0$ copies of unpaid (susceptible) node $\forall v \in V$, where $k_v$ are the number of paid (infected) neighbors (obtained from $\cM$). 
\item {\em Payment Scheduler:} A node $X$ selected is selected uniformly at random from $\cQ$ and added to the state memory $\cM$ (i.e., node $X$ gets its payment). All copies of $X$ are removed from $\cQ$ and one copy of each of $X$'s unpaid neighbors is added to $\cQ$.
\end{enumerate}
The following tables %~\ref{tab:desc} 
breaks down RW, SI, BFS, and DFS diffusion algorithms into their respective {\em pay-per-node} components (state memory, next-payment queue, payment scheduler).


%\begin{table}
%\caption{Diffusion Descriptions.}\label{tab:desc}
\begin{tabular}{ c l l l } 
\toprule
diffusion & next-payment queue & payment scheduler & state memory \\
\midrule
{\bf RW} & single node & - & no nodes \\
{\bf SI} & all covered unpaid & random order & all paid nodes \\
{\bf BFS} & all covered unpaid & FIFO & all paid nodes \\
{\bf DFS} & all covered unpaid & LIFO & all paid nodes \\
\bottomrule 
\end{tabular}
%\end{table}

Our metric of efficiency in {\em pay-per-node} diffusion is cover size $\vert \cI(n) \vert$ after $n$ payments. 
To illustrate our metric we compare $\vert \cI(n) \vert$ obtained with RWs, SI, BFS, and DFS on a real world network.
Fig.~\ref{fig:EnronBFS_SI} shows the {\em cover} set size on the Enron email network using BFS and SI.
OBSERVATIONS OF RESULTS.

\subsubsection{Optimal Solution}
The optimal cover size to a given budget is the Fractional Minimum Connected Dominating Set (FMCDS). The Minimum Dominating Set (MDS) is defined as the smallest set of nodes $D$, denotes the {\em cover set}, where all nodes in the graph are either in $D$ or are a neighbor of a node in $D$.
The Minimum Connected Dominating Set (MCDS) requires $D$ to form a connected component. 
And its fractional version FMCDS-$\epsilon$ relaxes the requirement that all nodes in the graph need to be covered for the requirement that just a fraction $\epsilon$ of the nodes need to be covered.
Section~\ref{sec:related} presents a literature review of the known FMCDS, MCDS, and MCS approximation algorithms and their guarantees.
For now it is important to stress that these approximation algorithms (most of them two-approximations) require node degrees to be known and, to the best of our knowledge, no approximation exists that assumes unknown node degrees.

The optimal solution to the MDS, however, provides us with an upper bound that can be used to compare algorithms.
That is, the maximum MCDS cover must be no smaller than the MDS cover.
INTEGER PROGRAM FORMULATION? DUALITY GAP? {\bf Approximability of power law graphs?}
Thus, two-approximations of the MDS cover can be used to find upper bounds to the MCDS cover.
Fig.~\ref{fig:ProgramAppx} shows

\begin{figure}
\centering
\includegraphics[width=3in,height=2in]{figs/effect_of_memory_Enron_ORIG}
\caption{Comparison of integer program MDS approximation, Max degree, Random Walks, BFS algorithms.\label{fig:ProgramAppx}}
\end{figure}



% Hence, degrees must be estimated from the current diffusion state. We conjecture that SI can be cast as a distributed stochastic algorithm that estimates the degree of an unvisited node from the current diffusion state and selects the next visited (infected) using a randomized variant of the Dual-fitting algorithm.

\begin{figure*}[t]
\centering
\includegraphics[width=3in,height=2.5in]{{{figs/effect_of_memory_Enron_ORIG+GSI.nodes}}}
~~~
\includegraphics[width=3in,height=2.5in]{{{figs/effect_of_memory_Enron_ORIG.nodes}}}
\caption{Cover versus Payments of na\"ive {\em pay-per-node} diffusions in the Enron email network.\label{fig:EnronBFS_SI}}
\end{figure*}






%The above are examples of information that can spread from person to person through like an epidemic through the network.
%Influenced by the idea of viral marketing campaigns, Domingos and Richardson~\cite{Domingos01,Richardson02}  and XXX considered the use of a set of highly influential people to maximize the number of infected nodes in the network.
%The search for such influential sets is a computationally difficult problem, although recent work has shown that when social influence follows the kind of ``diminishing returns'' pattern discussed here, it is possible to find approximate methods with provable guarantees by Kempe, Kleinberg, and Tardos~\cite{Kempe}.
% "Optimal marketing strategies over social networks" of \cite{Hartline08},  Eigenvalues of Graphs~\cite{Cristos}.
%
%The research community has mostly attacked the subject in essentially three fronts: {\em By measuring these epidemics in the wild} (e.g., \footnote{how the probability of purchasing books, DVDs, and music from a large online retailer increased with the number of email recommendations a potential customer received??? of Leskovec, Adamic, and Huberman~\cite{Leskovec07} and Backstrom et al. determined the probability of joining groups in a large online community as a function of the number of friends who already belonged to the group.4 And Hill, Provost, and Volinsky16 analyzed how an individualÕs adoption of a consumer telecommunications service plan depended on his or her connections to prior adopters of the service.While the probability of adopting a behavior increases with the number of friends who have already adopted it, there is a Òdiminishing returnsÓ pat- tern in which the marginal effect of each successive friend decreases.4,25 In many cases, however, an interest- ing deviation from this pattern is ob- servedÑa Ò0Ð1Ð2 effect,Ó in which the probability of joining an activity when two friends have done so is significantly more than twice the probability of joining when only one has done so.}), {\em by preventing bad ``information'' (a virus) to spread} (Cascading works), and {\em by helping unleash ``good'' contagion}, influenced by viral marketing strategies (e.g., the influence maximization  works of Domingos and Richardson~\cite{Domingos01,Richardson02}, Kempe, Kleinberg, and Tardos~\cite{Kempe}, and "Optimal marketing strategies over social networks" of \cite{Hartline08}, ~\cite{Cristos}.).
%
%3.	Domingos and Richardson [6, 18] are the first to study influence maximization as an algorithmic problem. Their methods are prob- abilistic, however. Kempe, Kleinberg, and Tardos [10] are the first to formulate the problem as a discrete optimization problem. Be- sides what we mentioned above already, they also study a number of other topics such as generalizations of influence cascade mod- els and mixed marketing strategies in influence maximization. As pointed out, a serious drawback of their work is the scalability of their greedy algorithm.
%4.	Several recent studies aimed at addressing this issue. In [14], Leskovec et al. present a Òlazy-forwardÓ optimization in select- ing new seeds, which greatly reduces the number of evaluations on the influence spread of nodes and results in as much as 700 times speedup demonstrated by their experimental results. However, even though the Òlazy-forwardÓ optimization is significant, it still takes hours to find 50 most influential nodes in a network with a few tens of thousands of nodes, as shown in [4].
%5.	In [11], Kimura and Saito propose shortest-path based influence cascade models and provide efficient algorithms to compute influ- ence spread under these models. The key differences between their work and ours are (a) instead of using maximum influence paths, they use simple shortest paths on the graph, which are not related to propagation probabilities, and (b) they do not utilize local struc- tures such as our arborescences and thus in every round they need global computations to select the next seed. Therefore, their algo- rithms are not scalable, as shown in our experiments.
%
%We refer broadly refer to the above research topics as {\em information diffusion}, where the contagion process is given to us.
%
%
%The possibility of artificially unleashing such cascades through clever seeding is of interest to the scientific community~\cite{Cristos,Etc} as well as marketing researchers~\cite{WiredMagazine?}.
%
%Models for the processes by which ideas and influence propagate through a social network have been studied in a number of do- mains, including the diffusion of medical and technological innova- tions, the sudden and widespread adoption of various strategies in game-theoretic settings, and the effects of Òword of mouthÓ in the promotion of new products. Recently, motivated by the design of viral marketing strategies, Domingos and Richardson posed a fun- damental algorithmic problem for such social network processes: if we can try to convince a subset of individuals to adopt a new product or innovation, and the goal is to trigger a large cascade of further adoptions, which set of individuals should we target?
%
%
%
%Epidemic seen as essentially a network discovery algorithm. In the classic Susceptible-Infected (SI) epidemic model each ``discovered'' (infected) node gets to participate in the network discovery process by infecting its neighbors~\cite{?}. SI together with a variety of different epidemic model have been throughly studied (we provide an overview in Section~\ref{?}).
%
%
%A novel research topic, that we briefly propose in this work, is the idea of {\em information propulsion}.
%In {\em information propulsion} information cascades are facilitated and possibly even controlled (engineered) by a set of agents that are either within or are external to the network.
%The social impact and implications of information diffusion and propulsion are indisputable.
%
%Despite the incredible strides that the independent study of {\em network searchability} and {\em information diffusion} has accomplished in the past years, we believe that until these phenomena are connected their understanding will remain incomplete.
%For one, {\em information propulsion} is missing in the picture.
%Moreover, evidence that high-degree nodes play an important role in both phenomena -- i.e., high-degree nodes shrinks network diameter in the search problem and facilitates the spread of information -- either tantalizingly indicates that these phenomena share common features or may be solely coincidental.
%We show that it is because search, diffusion, and propulsion are related that high-degree nodes play similar roles in these phenomena.
%To the best of our knowledge this work is the first to attempt such connection.
%

